DreamDrive: Generative 4D Scene Modeling from Street View Images

Synthesizing photo-realistic visual observations from an ego vehicle's driving trajectory is a critical step towards scalable training of self-driving models. Reconstruction-based methods create 3D scenes from driving logs and synthesize geometry-consistent driving videos through neural rendering, but their dependence on costly object annotations limits their ability to generalize to in-the-wild driving scenarios. On the other hand, generative models can synthesize action-conditioned driving videos in a more generalizable way but often struggle with maintaining 3D visual consistency. In this paper, we present DreamDrive, a 4D spatial-temporal scene generation approach that combines the merits of generation and reconstruction, to synthesize generalizable 4D driving scenes and dynamic driving videos with 3D consistency. Specifically, we leverage the generative power of video diffusion models to synthesize a sequence of visual references and further elevate them to 4D with a novel hybrid Gaussian representation. Given a driving trajectory, we then render 3D-consistent driving videos via Gaussian splatting. The use of generative priors allows our method to produce high-quality 4D scenes from in-the-wild driving data, while neural rendering ensures 3D-consistent video generation from the 4D scenes. Extensive experiments on nuScenes and street view images demonstrate that DreamDrive can generate controllable and generalizable 4D driving scenes, synthesize novel views of driving videos with high fidelity and 3D consistency, decompose static and dynamic elements in a self-supervised manner, and enhance perception and planning tasks for autonomous driving.

==> figs/algo.tex <==
\begin{algorithm}
\caption{\ourmethod{} Algorithm}
\begin{algorithmic}[1]

    \State \textbf{Input:} Control signals $X_{ctrl}$, e.g., single image $I_{ctrl}$, map with object locations $M_{ctrl}$.
    \State \textbf{Output:} 3D Gaussians $G: \{G_{static}, G_{dynamic}\}$ containing static and dynamic Gaussians.

    \State \hrulefill
    
    \State \textbf{Learning Phase:}

    \State $\{I_{ref}, Z_{ref}\} \gets F_{VDM}(X_{ctrl})$ \Comment{Video diffusion priors.}

    % \State \textbf{2. Geometry Initialization:}
    \State $\{G_{init}, P_{ref}\} \gets F_{MVS}(I_{ref})$ \Comment{Initializing 3D scene geometry and recovering camera poses.}
    
    \State \textbf{Optimize} $G_{init}$ assuming Gaussians are static.  

    \State \textbf{Optimize} $F_{cls}$ using the following loss:\\
    $I^t_{static} \gets F_{splat}(G_{init}, P^t_{ref})$\\
    $I^t_{err} \gets |I^t_{static} - I^t_{ref}|$ \\
    $S \gets F_{cls}(G_{init}, Z_{ref}).$\\
    $L_{dec} \gets \sum_{t=0}^T (L_{bce}(F_{splat}(S, P^t_{ref}), I^t_{err})).$

    \State \textbf{Decompose} $G_{init}$ into $\{G_{static}, G_{dynamic}\}$: \\
    $G^{\prime}_{dynamic} \gets \{G_{init} \mid S > \tau \}.$ \\
    $G^{\prime}_{static} \gets \{G_{init} \mid S \leq \tau \}.$\\
    $\{G_{static}, G_{dynamic}\} \gets F_{group}(G^{\prime}_{static}, G^{\prime}_{dynamic}).$

    \State \textbf{Optimize} $\{G_{static}, G_{dynamic}\}$ using the rendering loss: \\
    $I^t_{render} \gets F_{splat}(\{G_{static}, G^t_{dynamic}\}, P^t_{ref}).$ \\
    $L_{render} \gets \sum^T_{t=0} (L_{1}(I^t_{render}, I^t_{ref}) + L_{SSIM}(I^t_{render}, I^t_{ref})).$ 
    
    \State \hrulefill
    
    \State \textbf{Inference Phase:}
    
    % \State \textbf{1. 4D Scene Generation:}
    \State $\{G_{static}, G_{dynamic}\} \gets F_{gen}(X_{ctrl})$ \Comment{Generate the 4D scene using static and dynamic Gaussians.}

    % \State \textbf{2. Rendering:}
    \State \For{$t = 1$ to $T$}
        \State $I^t \gets F_{splat}(\{G_{static}, G^t_{dynamic}\}, P^t)$ \Comment{Render novel views at each timestep using learned Gaussians.}
    \EndFor
    \State \textbf{Output:} Driving video $V = \{I^t \mid t = 1, \dots, T\}$

\end{algorithmic}
\end{algorithm}


==> figs/control_method.tex <==
\begin{figure*}[htp]
    \centering
    \includegraphics[width=\textwidth]{figs/control_map_method.pdf}
    \caption{Your caption here}
    \label{fig:control_map_method}
\end{figure*}


==> tables/recon.tex <==
% this table can be removed

\begin{table}[th]
  \renewcommand{\arraystretch}{1.1}
  \renewcommand\tabcolsep{8.5pt} 
  \footnotesize
  \caption{4D Reconstruction quality of SynDrive against state-of-the-art methods. \yue{Like I siad, let's try to add more baselines here}}
    \vspace{-0.3cm}
    \begin{center}
    \begin{tabular}{l|cccc}
        \toprule[.03cm]
        Method & L1 $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
        \midrule
        3D-GS~\cite{3dgs} & 0.0178 & 29.0698 & 0.9198 & 0.0613 \\
        \ourmethod (Ours) & \textbf{0.0096} & \textbf{36.1912} & \textbf{0.9682} & \textbf{0.0185} \\
        \toprule[.03cm]
    \end{tabular}
    \end{center} 
    \label{tab:recon}
    \vspace{-0.7cm}
\end{table}


